Modelling and Optimisation of Resource Usage in an IoT Enabled Smart Campus

University campuses are essentially a microcosm of a city. They comprise diverse facilities such as residences, sport centres, lecture theatres, parking spaces, and public transport stops. Universities are under constant pressure to improve efficiencies while offering a better experience to various stakeholders including students, staff, and visitors. Nonetheless, anecdotal evidence indicates that campus assets are not being utilised efficiently, often due to the lack of data collection and analysis, thereby limiting the ability to make informed decisions on the allocation and management of resources. Advances in the Internet of Things (IoT) technologies that can sense and communicate data from the physical world, coupled with data analytics and Artificial intelligence (AI) that can predict usage patterns, have opened up new opportunities for organisations to lower cost and improve user experience. This thesis explores this opportunity via theory and experimentation using UNSW Sydney as a living laboratory.

==> tex/01-statements.tex <==
\newpage
\cleardoublepage
%==========================SIGNED DECLARATION==========================================================================
\clearpage
\thispagestyle{empty}
\includepdf[pages={1}]{unsw_documents/public/thesisdissertation_sheet}
\cleardoublepage

\clearpage
\thispagestyle{empty}
\includepdf[pages={1}]{unsw_documents/public/originalitystatement}
\cleardoublepage


\clearpage
\thispagestyle{empty}
\includepdf[pages={1}]{unsw_documents/public/copyrightauthenticitystatements}
\cleardoublepage

\clearpage
\thispagestyle{empty}
\includepdf[pages={1}]{unsw_documents/public/publicationsStatement}
\cleardoublepage

\chapter*{}
\thispagestyle{empty}
\vfil
\begin{center} To my family \end{center}
\vfil
\cleardoublepage


==> tex/02-lists.tex <==

%% TOC%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\tableofcontents
\cleardoublepage

\clearpage
\listoffigures
\cleardoublepage

\clearpage
\listoftables

\clearpage

\input{./sections/acronyms.tex}

==> tex/05-acronyms_old.tex <==
\newglossaryentry{x01}{ type=symbol, name=$G$,  description={Gravitational constant ($6.67408 \times 10^{-11}\ m^{3} kg^{-1}s^{-2}$)} }
\newglossaryentry{x02}{ type=symbol, name=$\mu_g$,  description={Standard gravitational parameter ($ m^{3}s^{-2}$)} }
\newglossaryentry{x03}{ type=symbol, name=$\mathit{r_i}$,  description={distance from $i^{th}$ octree node's centroid to external point (\textit{m})} }
\newglossaryentry{x04}{ type=symbol, name=$N$,  description={Number of octree nodes} }
\newglossaryentry{x05}{ type=symbol, name=$\vec{U}$,  description={Gravitational potential $ \in \mathbb{R}^1$} }
\newglossaryentry{x06}{ type=symbol, name=$\nabla \vec{U}$,  description={Gravitational acceleration $ \in \mathbb{R}^{3\times 1}$} }
\newglossaryentry{x07}{ type=symbol, name=$\nabla \nabla \vec{U}$,  description={Gravity gradient matrix \textit{or} Hessian of the potential  $ \in \mathbb{R}^{3\times 3}$} }
\newglossaryentry{x08}{ type=symbol, name=$\vec{r_i}$,  description={Vector from variable field point to polyhedron vertex} }
\newglossaryentry{x09}{ type=symbol, name=$\vec{E_e}$,  description={Edge dyad $ \in \mathbb{R}^{3\times 3}$} }
\newglossaryentry{x10}{ type=symbol, name=$\vec{F_f}$,  description={Face dyad  $ \in \mathbb{R}^{3\times 3}$} }
\newglossaryentry{x11}{ type=symbol, name=$L_e$,  description={Factor per-edge $ \in \mathbb{R}^1$} }
\newglossaryentry{x12}{ type=symbol, name=$\omega_f$,  description={Factor per-face  $ \in \mathbb{R}^1$} }
\newglossaryentry{x13}{ type=symbol, name=$ m $,  description={Mass ($kg$)} }
\newglossaryentry{x13a}{ type=symbol, name=$ M $,  description={Mass of a small body ($kg$)} }
\newglossaryentry{x14}{ type=symbol, name=$\rho$,  description={Density ($kgm^{-3}$)} }
\newglossaryentry{x15}{ type=symbol, name=$V$,  description={Volume ($m^{3}$)} }
\newglossaryentry{x16}{ type=symbol, name=$\mu$,  description={mean} }
\newglossaryentry{x17}{ type=symbol, name=$\sigma $,  description={standard deviation} }
\newglossaryentry{x18}{ type=symbol, name=$\textbf{\textsc{x}}_{s,a}^i$,  description={State at instance of time \textit{i}, $\left\lbrace i = 1, ..., N \right\rbrace$, subscript \textit{s}- spacecraft and \textit{a}-asteroid} }
\newglossaryentry{x19}{ type=symbol, name=$\vec{r}$,  description={position vector $ \begin{bmatrix} x & y & z \end{bmatrix}'$} }
\newglossaryentry{x20}{ type=symbol, name=$\vec{q}$,  description={quaternion $ \begin{bmatrix} q_0 & q_x & q_y & q_z \end{bmatrix}'$} }
\newglossaryentry{x21}{ type=symbol, name=$\vec{v}$,  description={velocity vector $ \begin{bmatrix} v_x & v_y & v_z \end{bmatrix}'$} }
\newglossaryentry{x22}{ type=symbol, name=$\bm{\omega}$,  description={angular velocity vector $ \begin{bmatrix} \omega_x & \omega_y &\omega_z \end{bmatrix}'$} }
\newglossaryentry{x23}{ type=symbol, name=${\vec{l}}_{k}^{i}$,  description={measurement of landmark \textit{k},  at instance \textit{i}; \textit{k} is the number of landmarks $ \left\lbrace k = 1, ..., M \right\rbrace $} } \newglossaryentry{x24}{ type=symbol, name=$\dotv{r}$, description={derivative of position} }
\newglossaryentry{x25}{ type=symbol, name=$\dotv{v}$, description={derivative of velocity} }
\newglossaryentry{x26}{ type=symbol, name=$\dotv{q}$, description={derivative of quaternion} }
\newglossaryentry{x27}{ type=symbol, name=$\dotv{\bm{\omega}}$, description={derivative of angular velocity} }
\newglossaryentry{x28}{ type=symbol, name=$J$,  description={Inertia matrix} }
\newglossaryentry{x29}{ type=symbol, name=$W(q)$,  description={quaternion rates matrix} }
\newglossaryentry{x30}{ type=symbol, name=$Q_v$,  description={process noise - including disturbance forces applied to the spacecraft} }
\newglossaryentry{x31}{ type=symbol, name=$Q_\omega$,  description={process noise - including disturbance torques applied to the spacecraft} }
\newglossaryentry{x32}{ type=symbol, name=$\mu$,  description={standard gravitational parameter} }
\newglossaryentry{x33}{ type=symbol, name=$\mathbf{r_c}$,  description={vector from the spacecraft to the asteroid's center of rotation} }
\newglossaryentry{x34}{ type=symbol, name=${r_k}$,  description={radius of the sphere formed by landmark \textit{k} during asteroid rotation  (scalar value)} }
\newglossaryentry{x35}{ type=symbol, name=$C_{nm}$,  description={dimensionless spherical harmonic  coefficients} }
\newglossaryentry{x35a}{ type=symbol, name=$S_{nm}$,  description={dimensionless spherical harmonic  coefficients} }
\newglossaryentry{x36}{ type=symbol, name=$P_{nm}$,  description={the Legendre polynomials $(m = 0)$ or associated Legendre functions $(m > 0)$ of degree $n$ and order $m$, $N$ is the maximum degree of the expansion} }
\newglossaryentry{x37}{ type=symbol, name=$E_n^m$,  description={$Lam\acute{e}'s$ function of degree $n$ and order $m$} }
\newglossaryentry{x37a}{ type=symbol, name=$F_n^m$,  description={$Lam\acute{e}'s$ function of degree $n$ and order $m$} }
\newglossaryentry{x38}{ type=symbol, name=$\alpha_n^m$,  description={dimensional coefficient equivalent to spherical harmonic coefficients $C_{nm}$ and $S_{nm}$} }
\newglossaryentry{x39}{ type=symbol, name=$C/N_0$,  description={Carrier-to-Noise density ratio (dB-Hz)} }
\newglossaryentry{x40}{ type=symbol, name=$EIRP$,  description={Equivalent isotropic radiated power (dB-W)} }
\newglossaryentry{x41}{ type=symbol, name=$G_t$,  description={Gain of transmission antennas (dB)} }
\newglossaryentry{x42}{ type=symbol, name=$G_r$,  description={Gain of receiving antennas (dB)} }
\newglossaryentry{x43}{ type=symbol, name=$L_f$,  description={Free space loss (dB)} }
\newglossaryentry{x44}{ type=symbol, name=$L_{atm}$,  description={Atmospheric loss (dB)} }
\newglossaryentry{x45}{ type=symbol, name=$K_B$,  description={Boltzmann constant (dBW/K-Hz)} }
\newglossaryentry{x46}{ type=symbol, name=$T_{sys}$,  description={System noise temperature (dB-K)} }
\newglossaryentry{x47}{ type=symbol, name=$P_{synodic}$,  description={Synodic period between the two satellites} }
\newglossaryentry{x48}{ type=symbol, name=$T_{user}$,  description={Orbital period of the user} }
\newglossaryentry{x49}{ type=symbol, name=$T_{GNSS}$,  description={Orbital period of the GNSS constellation} }
\newglossaryentry{x50}{ type=symbol, name=$\rho_{inner}$,  description={density of the inner octree nodes ($kgm^{-3}$)} }
\newglossaryentry{x51}{ type=symbol, name=$\rho_{outer}$,  description={density of the outer octree nodes ($kgm^{-3}$)} }

 
\newacronym{slam}{SLAM}{Simultaneous Localization and Mapping} 
\newacronym{nea}{NEA}{Near-Earth asteroids}
\newacronym{dor}{DOR}{Differential One-Way Ranging}
\newacronym{spc}{SPC}{Stereophotoclinometry}
\newacronym{lidar}{LIDAR}{Light Detection and Ranging}
\newacronym{fov}{FOV}{Field of View}
\newacronym{fft}{FFT}{Fast Fourier Transform}
\newacronym{fp}{FP}{Fixation Point}
\newacronym{lrf}{LRF}{Laser Range Finder}
\newacronym{imu}{IMU}{Inertial Measurement Unit}
\newacronym{icp}{ICP}{Iterative Closest Point}
\newacronym{edl}{EDL}{Entry, Descent, and Landing}
\newacronym{ard}{ARD}{Autonomous Rendezvous and Docking}
\newacronym{ais}{AIS}{Autonomous Inspection and Servicing}
\newacronym{ekf}{EKF}{extended Kalman Filter}
\newacronym{ukf}{UKF}{unscented Kalman filter}
\newacronym{cad}{CAD}{Computer Aided Design}
\newacronym{rbpf}{RBPF}{Rao-Blackwellised Particle Filter}
\newacronym{pnp}{PnP}{Perspective-n-Point}
\newacronym{sift}{SIFT}{Scalar invariant feature transform}
\newacronym{surf}{SURF}{Speeded-up Robust Feature}
\newacronym{brief}{BRIEF}{Binary Robust Independent Elementary Features}
\newacronym{orb}{ORB}{Oriented fast and Rotated BRIEF}
\newacronym{brisk}{BRISK}{Binary Robust Invariant Scalable Keypoints}
\newacronym{mser}{MSER}{Maximally Stable Extremal Regions}
\newacronym{ola}{OLA}{OSIRIS-REx Laser Altimeter}
\newacronym{tof}{TOF}{Time of Flight}
\newacronym{ourcvfh}{OURCVFH}{Oriented, Unique and Repeatable Clustered Viewpoint Feature Histogram}
\newacronym{isam}{iSAM}{incremental Smoothing and Mapping}
\newacronym{marco}{MarCO}{Mars Cube One}
\newacronym{aida}{AIDA}{Asteroid Impact and Deflection Assessment}
\newacronym{apex}{APEX}{Asteroid Prospection Explorer}
\newacronym{copins}{COPINS}{CubeSat Opportunity Payload Inter-satellite Network Sensors}
\newacronym{liaison}{LiAISON}{Linked Autonomous Interplanetary Satellite Orbit Navigation}
\newacronym{fdoa}{FDOA}{Frequency Difference of Arrival}
\newacronym{lvlh}{LVLH}{Local Vertical Local Horizontal}
\newacronym{srp}{SRP}{Solar Radiation Pressure}
\newacronym{anh3bp}{ANH3BP}{Augmented Normalized Hill Three-Body Problem}
\newacronym{heo}{HEO}{High Earth orbits}
\newacronym{leo}{LEO}{Low Earth Orbits}
\newacronym{meo}{MEO}{Medium Earth Orbits}
\newacronym{mom}{MoM}{Mars Orbiter Mission}
\newacronym{sbas}{SBAS}{Satellite-based Augmentation System}
\newacronym{pnt}{PNT}{Position, Navigation, and Timing}
\newacronym{gnss}{GNSS}{Global Navigation Satellite System}
\newacronym{waas}{WAAS}{Wide Area Augmentation System}
\newacronym{qzss}{QZSS}{Quasi-Zenith Satellite System}
\newacronym{egnos}{EGNOS}{European Geostationary Navigation Overlay Service}
\newacronym{gagan}{GAGAN}{GPS and GEO Augmented Navigation}
\newacronym{sdcm}{SDCM}{System for Differential Corrections and Monitoring}
\newacronym{tsv}{TSV}{Terrestrial Service Volume}
\newacronym{ssv}{SSV}{Space Service Volume }
\newacronym{ure}{URE}{User Range Error}
\newacronym{ecef}{ECEF}{Earth Centred Earth Fixed}
\newacronym{pdop}{PDOP}{Position Dilution of Precision}
\newacronym{igso}{IGSO}{Inclined geosynchronous orbit}
\newacronym{geo}{GEO}{Geostationary Earth Orbit}
\newacronym{gps}{GPS}{Global Positioning System}
\newacronym{glonass}{GLONASS}{GLObal'naya NAvigazionnaya Sputnikovaya Sistema}
\newacronym{irnss}{IRNSS}{Indian Regional Navigation Satellite System}
\newacronym{navic}{NAVIC}{NAVigation with Indian Constellation}
\glsaddall

\printglossary[style=super, type= symbol , nonumberlist]
\printglossary[style=super, type=\acronymtype, nonumberlist]

==> tex/nomenclature.tex <==
%% \chapter*{Nomenclature}
% \bookmarksetupnext{level=section}
% \addcontentsline{toc}{chapter}{Nomenclature}
% \onehalfspace
\mbox{}
% \setlength{\nomitemsep}{-\parsep}

\nomenclature{$G$}{Gravitational constant ($6.67408 \times 10^{-11}\ m^{3} kg^{-1}s^{-2}$)}
\nomenclature{$\mu_g$}{Standard gravitational parameter ($ m^{3}s^{-2}$)}
\nomenclature{$\mathit{r_i}$}{distance from $i^{th}$ octree node's centroid to external point (\textit{m})}
\nomenclature{$N$}{Number of octree nodes}
\nomenclature{$U$}{Gravitational potential $ \in \mathbb{R}^1$}
\nomenclature{$\nabla U$}{Gravitational acceleration $ \in \mathbb{R}^{3\times 1}$}
\nomenclature{$\nabla \nabla U$}{Gravity gradient matrix \textit{or} Hessian of the potential  $ \in \mathbb{R}^{3\times 3}$}
\nomenclature{$\vec{r_i}$}{Vector from variable field point to polyhedron vertex}
\nomenclature{$\vec{E_e}$}{Edge dyad $ \in \mathbb{R}^{3\times 3}$}
\nomenclature{$\vec{F_f}$}{Face dyad  $ \in \mathbb{R}^{3\times 3}$}
\nomenclature{$L_e$}{Factor per-edge $ \in \mathbb{R}^1$}
\nomenclature{$\omega_f$}{Factor per-face  $ \in \mathbb{R}^1$}
\nomenclature{$ m $}{Mass ($kg$)}
\nomenclature{$\rho$}{Density ($kgm^{-3}$)}
\nomenclature{$V$}{Volume ($m^{3}$)}
\nomenclature{$\mu$}{mean}
\nomenclature{$\sigma $}{standard deviation}
\nomenclature{$\textbf{\textsc{x}}_{s,a}^i$}{State at instance of time \textit{i}, $\left\lbrace i = 1, ..., N \right\rbrace$, subscript \textit{s}- spacecraft and \textit{a}-asteroid}
\nomenclature{$\vec{r}$}{position vector $ \begin{bmatrix} x & y & z \end{bmatrix}'$}
\nomenclature{$\vec{q}$}{quaternion $ \begin{bmatrix} q_0 & q_x & q_y & q_z \end{bmatrix}'$}
\nomenclature{$\vec{v}$}{velocity vector $ \begin{bmatrix} v_x & v_y & v_z \end{bmatrix}'$}
\nomenclature{$\bm{\omega}$}{angular velocity vector $ \begin{bmatrix} \omega_x & \omega_y &\omega_z \end{bmatrix}'$}
\nomenclature{${\vec{l}}_{k}^{i}$}{measurement of landmark \textit{k},  at instance \textit{i}; \textit{k} is the number of landmarks $ \left\lbrace k = 1, ..., M \right\rbrace $}
\nomenclature{$\dotv{r}, \dotv{v}$}{derivative of position \& velocity}
\nomenclature{$\dotv{q}, \dotv{\bm{\omega}}$}{derivative of quaternion \& angular velocity}
\nomenclature{$J$}{inertia matrix}
\nomenclature{$W(q)$}{quaternion rates matrix}
\nomenclature{$Q_v, Q_\omega$}{process noise models including disturbance forces, torques applied to the spacecraft}
\nomenclature{$\mu$}{standard gravitational parameter}
\nomenclature{$\mathbf{r_c}$}{vector from the spacecraft to the asteroid's center of rotation}
\nomenclature{${r_k}$}{radius of the sphere formed by landmark \textit{k} during asteroid rotation  (scalar value)}
% \nomenclature{}{}
% \nomenclature{}{}
% \nomenclature{}{}


\printnomenclature
